Network Function Capacity Reconnaissance by Remote Adversaries

There is anecdotal evidence that attackers use reconnaissance to learn the capacity of their victims before DDoS attacks to maximize their impact. The first step to mitigate capacity reconnaissance attacks is to understand their feasibility. However, the feasibility of capacity reconnaissance in network functions (NFs) (e.g., firewalls, NATs) is unknown. To this end, we formulate the problem of network function capacity reconnaissance (NFCR) and explore the feasibility of inferring the processing capacity of an NF while avoiding detection. We identify key factors that make NFCR challenging and analyze how these factors affect accuracy (measured as a divergence from ground truth) and stealthiness (measured in packets sent). We propose a flexible tool, NFTY, that performs NFCR and we evaluate two practical NFTY configurations to showcase the stealthiness vs. accuracy tradeoffs. We evaluate these strategies in controlled, Internet and/or cloud settings with commercial NFs. NFTY can accurately estimate the capacity of different NF deployments within 10% error in the controlled experiments and the Internet, and within 7% error for a commercial NF deployed in the cloud (AWS). Moreover, NFTY outperforms link-bandwidth estimation baselines by up to 30x.

==> 2b.tex <==
\section{Prior Work and Limitations}
\label{sub:overview}

Even with our scoped problem definition, inferring capacity is challenging. %as we discuss next. %To show this, we walk through the potential steps of an attacker aiming at estimating the capacity of \NF to optimize her later attack. 
A natural starting point for an attacker is to use link-bandwidth estimation techniques to find the bandwidth of a bottleneck link.  Depending on the probing technique, the signal measured, and measurement requirements, these techniques can be grouped into three categories: \\
\myitem{Dispersion-based} techniques typically send a sequence or pair of packets and measure the spacing at the receiver~\cite{carter1996measuring,jacobson1997pathchar,li2008wbest}. \\ \myitem{Rate-based} techniques iteratively probe at increasing rates until the measured one-way-delay increases signalling self-induced congestion~\cite{ribeiro2003pathchirp,jain2002end}. \\
   \myitem{Bulk-transfer} techniques send a high volume of traffic for a longer duration and measure throughput (\ie after self-induced drops) at the receiver~\cite{tirumala1999iperf,allman2001measuring}.

%\end{packeditemize}

%that we are considering to make the problem tractable (\S~\ref{ssec:problemscope}).
%Next, we provide an overview of our design. namely \sys and explain how it navigates the challenges we reviewed in \S\ref{ssec:challenges}.

% \renewcommand{\arraystretch}{1.2} 
% // (or 1.3)
\begin{table}[t!]
\small
    \centering
    \begin{tabular}{@{}p{2cm}p{1.9cm}p{2cm}p{2cm}@{}} 
    \toprule
     Techniques & Low Network Footprint & Insensitive to Server Config. & Measurement Requirements\\
    \midrule
   \mbox{Dispersion-based}  & \cmark & \xmark & \timestamps\   \fastsending  \\
    \mbox{Rate-based}    & \xmark & \xmark & \timestamps\ \fastsending\  \precisesending \\
    \mbox{Bulk-Transfer} & \xmark & \cmark & \accuratecapturing  \\
    \multicolumn{4}{l}{\footnotesize \timestamps  = Accurate timestamping at the receiver, \fastsending  = Fast packet } \\ \multicolumn{4}{l}{\footnotesize generation at the sender, \accuratecapturing = Accurate capturing at receiver } \\
    \multicolumn{4}{l}{\footnotesize \precisesending  = Fine-grained control over send rate at the sender }\\
    \bottomrule
    \end{tabular}
    \caption{Summary of the bandwidth-estimation techniques in terms of their network footprint, ability to accommodate the server configurations, \& measurement requirements.}
    \label{tab:be-tech}
\end{table}
%\subsection{Bandwidth estimation approaches do not apply}\label{ssub:challenges}
% \aqsa{I would change bandwidth estimation to Naive/Existing approaches do not work and then change the next heading to flooding is accurate but visible, instead of rate based techniques.}




%In doing so, we also discuss why the most relevant previous work, namely link bandwidth estimation techniques are not applicable.

Next, we discuss why existing approaches are insufficient in the context of our  (scoped) \NFCR problem.  Table~\ref{tab:be-tech} summarizes these techniques and how they may apply to our \NFCR context. 

%\myitem{An attacker that floods the \NF can accurately estimate its capacity but is highly visible.} 

\myitem{Bulk-transfer techniques are accurate but detectable. }
An attacker might try to flood the \NF by sending packets at a high rate and measure the arrival rate at the receiver to find the \NF's true capacity. %To that end, the attacker would send at a high rate (in-bulk) for a few seconds and measure the arrival rate at the receiver. The received rate would naturally correspond to the maximum capacity of the \NF. 
While accurate, this is not suitable for \NFCR  as it would be easily detectable. Other techniques like Pathload~\cite{jain2002end} that send multiple batches of packets at increasing rates also have a high network footprint.  %Indeed, as they iteratively send at increasing rates and only terminate the search after they have exceeded the \NF's capacity, their aggregate network footprint will also be prohibitively high.

\remove{
\begin{table}[t!]
    \centering
    \begin{tabular}{ccc}
         & Packet Pair & Flooding\\
         \midrule
      \surrl   & 10 & 1406400 \\
      \surbl & 10 & 1164600 \\
      \snortrl & 10 & 634200 \\
      \bottomrule
    \end{tabular}
    \caption{Flooding has very high network footprint independently on the \NF. }
    \label{tab:pkt-ex}
\end{table}
}
%Naturally, this was not a critical requirement for link bandwidth estimation, hence was not considered by previous works.


%\myitem{An advanced attacker that uses  packet-spacing (dispersion) can be invisible but but cannot accurately estimate the NF's capacity.} 
\myitem{Packet-spacing (used in dispersion-based techniques) is stealthy but may be inaccurate.} 
The link-bandwidth estimation literature proposes more complex techniques than bulk-send~\cite{jacobson88congestion,bolot1993characterizing,carter1996measuring,dovrolis2001packet,jain2002end,kapoor2004capprobe,lai1999measuring,paxson1997end}, which  can, in theory,  estimate the \NF capacity. In practice, though, such techniques do not work for \NFCR. We find empirically that they result in highly inaccurate capacity estimations. As an illustration, Figure~\ref{fig:fs-ex} compares bulk-send and packet pair (a well-established dispersion-based bandwidth-estimation technique) in estimating the capacity of three realistic \NFs. We use the bulk-send approach for the ground-truth capacity as it resembles an actual attack. We see that the packet-pair technique results in  high inaccuracy (up to 65\% error).  Investigating this  further, we found that it stems from two main reasons: \emph{(i)} measurement inaccuracies; and \emph{(ii)} server-side optimizations to reduce energy consumption (e.g., DVFS). 
%Importantly, this observation is not particular to packet-spacing. 
%As such optimizations are not used in links, all link capacity estimation techniques (beyond flooding) would result in highly inaccurate results when used for \NF estimation.



\begin{figure}[t!]
\small
    \centering
    \includegraphics[width=0.75\columnwidth]{fig/fs-ex.png}
    \caption{The bulk-transfer technique results in more accurate capacity estimation compared to packet pair.}
    \label{fig:fs-ex}
\end{figure}


%\myitem{All techniques fail unless the measurement infrastructure is fine-tuned.}
\myitem{All estimation techniques fail without accurate, fine-grained, and noise-free measurements.} The accuracy of different bandwidth-estimation techniques~\cite{carter1996measuring,lai1999measuring,lai2001nettimer,dovrolis2001packet,johnsson2004diettopp}, regardless of the metrics they measure, are affected by various underlying factors that are often not considered.   
%Importantly, most of these factors have been under-looked by previous work on bandwidth estimation\cite{carter1996measuring,lai1999measuring,lai2001nettimer,dovrolis2001packet,johnsson2004diettopp}.
For example, one-way delay used by some techniques~\cite{kapoor2004capprobe} is affected by clock drift.
%synchronization issues, thus the attacker would require to often sync the sender and receiver. 
Similarly, packet spacing is affected by different Internet paths or multi-queue NICs, causing packet re-ordering. Finally, these strategies are affected by batching at the receiver either in software (NAPI~\cite{salim2001beyond}) or hardware(IC~\cite{IC}), leading to inaccurate timestamps. 
% \maria{@aqsa can you check that this is in sync with the table?}

%Any strategy would be affected by bathing at the receiver either in software (NAPI~\cite{}) or in hardware(IC~\cite{}). 

%Measuring one-way-delay, round-trip-time, packet spacing, \etc is essential for any cap technique but affected by various factors. 

%An attacker might try to send at various rates and measure the increases in the one-way-delay would indicate congestion. Unfortunately, this would not work because of the lack of syncronization, FS on the sender and granularity at the receiver side.

\myitem{Bandwidth estimation  entails  two-sided control.}
Most traditional bandwidth estimation techniques assume two-sided control of the link.  %\ie assume the attacker controls two vantage points: before and after the link of interest. 
%Extending the existing approaches is non-trivial. 
Furthermore, bandwidth estimation techniques that do not assume two-sided control do not work for a one-sided \NFCR. In those techniques, the reply is sent via a public server which is triggered by a particular packet type (\eg a TCP SYN on a closed port triggers a TCP RST~\cite{saroiu2002sprobe} or an ICMP ECHO request triggers an ICMP reply~\cite{carter1996measuring}). Unfortunately, these packet types might not be processed by the \NF of interest (\eg a SYN proxy will not process an ICMP ECHO request). 

%\aqsa{I think we should give an actual example here. No BE technique uses HTTP. they either use TCP SYN/RST or ICMP ECHO/REPLY. Possible solution: In those techniques reply assumes a particular protocol behavior such as TCP SYN/RST. Indeed, these packet types might not be processed by the \NF of interest (\eg a UDP firewall will not process a TCP SYN packet.)}
%As an intuition, while one could, in theory, trigger a reply from routers in the path the measurements will be highly noisy \eg due to the router's load, and processing times.


%rate-limiting of such packets. For example, in our experiments, we tried three routers in the university network and found that two of them rate limited packets at 5 packets per second.\maria{what about the other two?} This is in sync with the extended study of Ravaioli\etal~\cite{ravaioli2015characterizing} %characterized ICMP rate 
%who found that 60\% of the routers implemented ICMP TTL Exceeded rate limiting. 




%\begin{tcolorbox}[colback=grey!5!white,colframe=black!75!black,boxrule=0.75pt]
%\textbf{Takeaway:} Bandwidth estimation techniques are not adequate for NF Capacity Reconnaissance (\NFCR). Indeed, BE techniques often have a high network footprint, do not trigger full capacity exposure and do not work beyond two-sided control. Among the alternatives, dispersion-based techniques appear to  more promising for \NFCR due to its low network footprint.

%\end{tcolorbox}



%existing bandwidth estimation techniques fail because they either have a high network footprint which makes the attack easily detectable. 
%Techniques with a lower network footprint are inaccurate because of server-side optimizations to reduce its energy consumption, and because of measurement inaccuracies. 
%Moreover, existing bandwidth estimation techniques pose two sided control as a hard requirement. 



==> 4-overview.tex <==


\section{\sys overview}

In this section, we give an overview of \sys and describe its most critical design decisions via intuitive examples. Consider an attacker that aims to estimate the maximum packet processing rate of an NF for a particular packet type (e.g. UDP). The NF is deployed at the edge of a victim network (as in Fig.~\ref{fig:setting}). The attacker might control the sender only (one-sided threat model) or both sender and receiver (two-sided threat model). 
% \aqsa{Not true b/c in one sided sender is also the receiver, we should say single node in the internet when referring to one-sdied
% }
To this end, the attacker sends a set of UDP packets to a host such that they are processed by the NF. To remain stealthy, the attacker does not flood the NF or use rate-based iterative probing. Instead, the attacker measures the dispersion \ie the NF-induced time gap between consecutive packets to infer the NF processing capacity. After being processed by the NF the packets will be spaced out in time depending on the NF processing time (Figure \ref{fig:disp}). 
The attacker manages to cause the \NF to run at its maximum (true) rate, while staying under the radar.% by sending a packet burst. 
The burst instantaneously stresses the \NF and creates a clear step-wise  pattern in the dispersion values that the attacker can recognize and use to find the true capacity.
We elaborate on how the attacker adapts traditional dispersion-based techniques to the \NFCR context in \S\ref{sec:dispersion}.
%and \S \ref{sec:estimation}. %At a high level, the attacker needs to \emph{(i)} trigger the NF's true capacity; 
%and \emph{(ii)} reduce noise from network and system's infrastructures. To that end, the attacker sends a burst of packets that instanteneusly

%To be more stealth, the \sys attacker uses dispersion over rate-based techniques. As rate-based techniques rely on iterative probing involving self-induced congestion to adapt their sending rate, they are strictly more visible than dispersion based approaches which rely on a single probe  (\S\ref{sec:dispersion}). 

If the attacker is two-sided \ie controls a receiver, the attacker measures the packet dispersion directly ( Fig.\ref{fig:disp}). If the attacker is one-sided, she engineers a subset of the sent packets to trigger an error message from an on-path router after the NF. Next the one-sided attacker measures the dispersion between consecutively received error messages (\S\ref{sec:onesided}). As an illustration,  Fig. \ref{fig:router-processing} shows an one-sided attacker that triggers the router to send a TTL time exceeded error message (after processing by the NF) back to the sender. Notably, \sys does not need to receive trigger engineer all packets to return as error messages.

\sys generalizes to multiple NFs and deployments and is configured with two parameters: \emph{(i)} the number of packets it sends; and \emph{(ii)} (for one-sided only) the gap between packets that trigger a router in the path. 
Intuitively, sending more packets allows for higher accuracy as it triggers the NF's true behavior, but makes the attack more detectable. We analytically and experimentally find the minimum  number of packets that need to be sent to accurately estimate an NF's capacity. We discuss our findings in (\S\ref{sec:e2e}) and summarize our results in a decision tree in Fig.\ref{fig:decision-tree}.


%To trigger the NF's true capacity, the \sys attacker sends a burst of packets targeting a host inside the victim network, (DVFS, multi threading \etc). Next the attacker, processes the measured dispersion to produce the final capacity estimate considering DVFS, multi-threading \etc (\S\ref{sec:length}). 

 


% \subsection{Overview}
%\sys is based on three key design decisions. 
%First, \sys uses dispersion over rate-based techniques. As rate-based techniques rely iterative probing involving self-induced congestion to adapt their sending rate, they are strictly more visible than dispersion based approaches which rely on a single probe. 
%Second, to trigger the NF to run at its full capacity, \sys sends more packets (than traditional techniques) as fast as possible and uses different packet headers \aqsa{i think we should write flows here different packet headers is too open.}. Doing so triggers DVFS and utilizes all threads.
%Third, to make the attack effect with one-sided control \sys sets TTL to lower bits to trigger TTL expired messages which act as replies. 








%Given our analysis of prior work, we revisit the problem of \NFCR from first principles and observe that any design needs to address  challenges on two fronts:  \textbf{probing strategy} and \textbf{measurement infrastructure}. The probing strategy includes the type and rate of packet probes, the measured signal, and the processing of the measurements. The measurement infrastructure refers to tools for packet capture, sending traffic, and system configurations of the sender and receiver. 

%(Note that depending on the one- or two-sided model the location of the receiver could differ.) 

%Given this abstract view, we can now attribute the limitations of the existing tools to both  probing- and measurement-related issues.
%These are  hard to address and can cause the \NFCR to fail.
%For example, a poor probing strategy will result in an easily detectable or inaccurate \NFCR.
%For example, a rate-based probing strategy might flood the \NF making 
%the \NFCR detectable. Similarly, a probing strategy that is not resilient to noise (e.g., due to hardware or  congestion) will lead to an inaccurate estimation.
%At the same time, poor measurement infrastructure can also result in  biased and noisy estimation; e.g.,  if the attacker's packets take different Internet paths or if the sending rate is too slow.

%, the measurements will be noisier, making any inference less likely to succeed. 
%Similarly, if the sender does not send packets fast enough, she might never reach the \NF's limits, leading the attacker into believing that the \NF has ahttps://www.overleaf.com/project/61e4e1c025dbc95a5241cd09 lower capacity.


%These above issues  are merely illustrative. 
%and  barely scratch the surface of challenges that can ruin the \NFCR effectiveness as we will see next. %Worse yet, 
%In the rest of the paper, we analyze the challenges and systematically walk through our design choices to realize \sys. 
%through our design process in realizing \sys,  a novel \NFCR system.  
%For clarity, we start with the two-sided threat model where the attacker controls two vantage points such that the generated traffic passes via the \NF  (\S\ref{sec:design}, \S\ref{sec:measurements}). In \S\ref{sec:design}, we discuss the trade-offs in different probing strategies and estimation functions given the probing results. 
 %Once we construct the \sys probing strategy, in \S\ref{sec:measurements}, we describe and address the requirements that this strategy imposes on the measurement infrastructure. 
%Then, we  extend this basic framework to  the one-sided model  (\S\ref{sec:onesided}). %\vyas{feel like this para needs to come earlier?}


 
%and risks of different probing interarrival rates, from sending a single packet pair to sending in bulk. 
%We explain how measuring the spacing between packets can give us an accurate estimation of the capacity of the \NF.
 %We also discuss the effectiveness of measuring different signals, from one-way delay to packet spacing. Finally, we discuss the effectiveness of different functions in post-processing the measurements to reduce the noise and trigger more accurate estimation. 
  
%Concretely, we explain the requirements of the sending rate and the timestamping granularity. We also explain the hardware and software means that we can use to achieve them from both the sender's and the receiver's perspective.




%In \S~\ref{}, we discuss the unique challenges that the single-sided threat model brings. We find their root causes and we describe \sys approach to address them.




%\sys, namely a technique for solving the problem we defined in~\S~\ref{ssec:problemscope}. In this section we present a running example of \sys, before we explain the trade-offs and reasoning of each of our design decisions in \S~\ref{sec:design}









%\vyas{Mar 31: Here is my suggestion to this section. Extend 4 to raise three types of challenges: PRobe DEsign, MEasurement Design, One sided Design prefetching a subset of the qns from current 5. Then setup a roadmap for the reader -- we will start with the two sided model and describe the probe and meausrement infr and then discuss e4xtension to one sided. so id have three small sections -- probe, measurement, one sided extension. having a huge monolithic 5 makes readability hard} 


%\maria{Designing a \NFCR attack constitutes in constructing three key components that address sensing, analysis and actuation. 
%From the sensing perspective an attacker needs to decide the rate and type of packets she will use to probe (sense) the \NF. 
%Sensing is an online operation and aims at maximizing the fidelity of the measurements while keeping the \NFCR under the radar.
%From the analysis perspective an attacker needs to decide how to processes the collected data.
%Analysis is an offline process and aims at minimizing the effect of noise in the inferred capacity .
%Finally, from the actuation perspective an attacker needs to decide what measurement infrastructure needs to be used to accurately instantiate the sensing and analysis design goals. Actuation is online and limited by the attackers access.}



\remove{

To describe \sys we provide our key insights for constructing the inference model.
We answer three key questions: \emph{(i)} what \sys measures; \emph{(ii)} what it its probing strategy; \emph{(iii)} how it analysis the measurement; \emph{(iv)} how it can be extended to a single-sided attacker.

\myitem{\sys measures packets spacing (dispersion) to reduce the attacker's footprint.}
Rate-based and Bulk-transfer techniques fail in \NFCR because they generate a lot of traffic as shown in Fig.~\ref{fig:fs-ex}.
To avoid this, \sys uses packet dispersion, that is, \emph{(i)} the sender VP sends a train of packets \emph{(ii)} the \NF processes these packets one-by-one; \emph{(iii)} the receiver captures them and reports the time difference between packets. 
\aqsa{its repetitive after the examples}
The measured time differences (dispersion) correspond to the time the \NF took to process each packet, we elaborate on this in \S~\ref{} .
To prevent the packets from taking different paths (\eg guided by multi-queue NICs or load balancing), \sys generates trains of packets that correspond to the same flow. 
As dispersion, relies on measuring the time \NF takes to process a packet rather than the rate after which the \NF fails, it does not need to induce congestion\aqsa{we do induce congestion}, effectively incurring a smaller network footprint compared to other techniques.
\aqsa{Perhaps we can say: As dispersion, relies on measuring the time \NF takes to process a packet rather than the rate after which the \NF is saturated, it does not need to iteratively probe to converge on the minimum rate that causes congestion. Hence, dispersion-based techniques effectively incur a smaller network footprint as compared to other techniques.}


%\myitem{I2: Use large packet trains reveal server capacity while staying under budget.}
%add generality i.e. one could try to profile each different MF independently 
%The most straightforward way to measure the capacity of an \NF is flooding the \NF with packets until it becomes in-responsive. 
%Multiple optimizations might affect the observed server capacity. We noticed that the measured processing capacity often changes as the load on the server increases. 



\myitem{\sys sends once a probe of full-budget size to maximize the information gain.}
Naively sending small trains, as done in traditional network bandwidth estimation techniques~\cite{lai1999measuring, dovrolis2001packet}, is destined to be inaccurate due to the software adaptations of the offered capacity according to seen load. 
As an illustration, Figure~\ref{fig:large-trains} shows the observed dispersion as a function of the train size (number of packets in train). 
The real capacity is revealed only after $800$ packets. Of course, the exact number of packets that are required before this transition is unknown.
Thus, to maximize \sys's chances of observing the true capacity while staying within budget, \sys sends a  train of \trainsize packets where \trainsize is equal to our budget \budget.


\myitem{\sys locates a window of the most reliable measurements via a step detection technique.}
After receiving the train of packets, the attacker  needs to infer a single value to use across all packet dispersion values. Importantly, not all values are correct and naively selecting one say the minimum dispersion  will make the technique extremely sensitive to noise caused by congestion.
To address this challenge, \sys uses a well-established statistical method \stepDetectionAlgo~\cite{truong2020selective} for step detection to ensures that it considers the correct window of values. 
For instance, in the case of  Figure~\ref{fig:large-trains}, \sys will make sure that it only considers measurements after the $800$-th packet. 
We provide more details on how we make this process more general in \S~\ref{}

% consecutive packets and measures their inter-arrival gap between their being processed by the mitigation function.


%\todo{Add accuracy in sending, if we don't bypass the kernel our train will not be queued (?)}
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.9\columnwidth]{fig/large-trains.pdf}
    \caption{Sending large trains (multiple back-to-back packets) triggers frequency scaling.}
    \label{fig:large-trains}
\end{figure}

\maria{Consider removing it}
\myitem{\sys has a robust measurement infrastructure without using specialized hardware.}
\sys's design decisions guide the selection of measurement tools that minimizes the effect of noise from various sources \eg server configuration, hardware limitations \etc.
As an intuition, \sys uses DPDKcap to bypass the kernel, thus avoid the effects of interrupt throttling and other kernel induced noise.
The use of dispersion alleviates the need for syncing clocks between sender and receiver, which is hard to do at microsecond granularity without specialized hardware~\cite{yin2016can}.
The use of large trains minimizes the effects of DVFS at the receiver and sender.


%\myitem{Ensure accurate measurements.} 
%As today's \NF are extremely fast \ie few decades of $\mu$ the accuracy of the attacker's measurement infrastructure is critical. Among others, we found that batching can further decrease the accuracy.
%Thus, we build \name on top of dpdk-cap.


%\myitem{Account for server configurations}


%\myitem{Account for network congestion}
%If there is network congestion after the mitigation function, the dispersion might be smaller or larger than the ground truth.





\begin{figure}[t!]
    \centering
    \includegraphics[width=0.9\columnwidth]{fig/router-processing.pdf}
    \caption{
    In one-sided threat model, the router's processing overhead for ICMP replies may change the spacing across packets (dispersion), effectively ruining the signature.
   % The figure shows that in one sided control, when the TTL of packets expire at the router, the router may take longer time than the \NF to process the ICMP TTL Exceeded reply, thus interfering with the dispersion signature from the \NF.
    }
    \label{fig:router-processing}
\end{figure}

\myitem{\sys works under the one-sided model by infrequently triggering a router's reply.}
\name exploits the \emph{ICMP time exceeded} messages sent as error messages from routers to hosts upon receiving a packet that has no time to reach its destination. Such a solution is not trivial, though, due to the processing time at the router and the rate-limiting of such packets as shown in Figure~\ref{fig:rate-limiting}. For example, in our experiments, we tried three routers in the university network and found that two of them rate limited packets at 5 packets per second. This is in sync with the extended study of Ravaioli\etal~\cite{ravaioli2015characterizing} %characterized ICMP rate 
who found that 60\% of the routers implemented ICMP TTL Exceeded rate limiting. 
%\todo{A figure for this challenge?}

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width=0.9\columnwidth]{fig/rate-limiting.pdf}
%     \caption{The figure illustrates how ICMP ratelimiting can result in missing probes in one-sided \sys}
%     \label{fig:my_label}
% \end{figure}




\remove{
\begin{enumerate}
    \item \textbf{Accurate measurements} with dpdk-cap and accurate time-stamping.
    \item \textbf{Robust to server configurations } with adequately large train sizes.
\item \textbf{Rubust to network congestion} with selecting the minimum dispersion value. \aqsa{I think this is not unique to server capacity estimation. What we could contribute here is if we try to collect measurements from different vanatage points, noting that some path from a given vanatage point may not be congested. and this will also be different from link capacity estimation because there we cannot do this. }
\item \textbf{Minimize probability of detection by sticking to the budget}.
\end{enumerate}
}



\remove{
In this subsection, we review literature work on remote bottleneck estimation. We first briefly summarize their approaches and then explain they cannot satisfy the requirements.

\myitem{Server Bottleneck Estimation}
There have been efforts to remotely estimate bottlenecks of servers.
Among those Ramamurthy et~al.~\cite{ramamurthy2008remote} was not designed to target   describe an method that sends mini flash crowds \ie is a surge in traffic towards a server and estimates various bottlenecks such as access bandwidth, CPU utilization, memory usage.

by observing the delay after saturation. 
This is not directly applicable to our case because processing capacity of mitigation modules in a DDoS defense system is designed to receive huge loads. In effect, saturating such system requires  sending huge flash crowds, and risk detection.

\myitem{Link Bandwidth Estimation}
There have been efforts to remotely estimate the bottleneck link bandwidth, and available bandwidth of a path. We categorize them into three categories:

\begin{enumerate}
    \item Variable packet sizing (VPS): VPS techniques rely on the fact that link delays change with packet sizes, which does not apply to processing capacity.
    \item Statistical Traffic Modeling: These techniques use statistical or stochastic models for traffic to estimate the link bandwidth. These models often make strong assumption about the traffic and hence are inaccurate in realistic scenarios.
    \item Probe rate models: SLDRT, SLoPS, ToPP, PathCos, etc. These techniques rely on sending a lot of packets at varying rate to induce congestion in the bottleneck link and then by looking at the one way delay, they estimate the bandwidth. This probing nature of these techniques will raise alarm at the defense system.
    \item Dispersion based techniques: These techniques build on packet-pair probing. Packet pair probing does not involve sending too many packets and hence it fulfils our requirements.
\end{enumerate}
% using techniques such as variable packet sizing (VPS), packet pair probing, self loading periodic streams (SLoPS) etc. Some of these techniques cannot be applied to infer packer processing capacity such as  Similalry, SLoPS require sending a lot of packets at varying rate to learn the available bandwidth, which will raise alarms at the defense system. Packet pair probing on the other hand can be used to estimate the packet processing time from which we can estimate the processing capacity. However, packet pair probing fails in the presence of congestion either on the path or in the mitigation function~\cite{}, and it does not work in case of a multi-threaded mitigation function. 


Server Bottleneck Estimation e.g., Ramamurthy et~al. ~\cite{ramamurthy2008remote}, SLoPS~\cite{jain2002end,ribeiro2003pathchirp} require sending a lot of packets at varying rate to learn the available bandwidth, which will raise alarms at the defense system.
Other examples: PathChrip, ToPP, SLDRT etc.



Previous methods either make strong assumptions about cross-traffic and network delays \eg~\cite{Delphi,kelly}

Variable packet sizing (VPS)\cite{jacobson1997pathchar,lai2001nettimer} does not solve our problrm because it relies on the fact that link delays change with packet sizes, which does not apply to processing capacity. 



% \myitem{Stochastic Modeling}
% Another way to estimate the packet processing capacity of the mitigation module of a defense system would be to use queuing theory and model the mitigation module e.g., as an M/M/1 queue to reason about its processing capacity~\cite{} based on its processing time. However, this approach assumes that we control all the traffic entering the mitigation function, and also know about all the other network delays such as transmission delay etc. which is not realistic. 

% \myitem{Link Bandwidth Estimation}
remotely estimate the bottleneck link bandwidth, and available bandwidth of a path using techniques such as variable packet sizing (VPS), packet pair probing, self loading periodic streams (SLoPS) etc. rely on the fact that link delays change with packet sizes,








\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{fig/unoptimized baselines.png}
    \caption{The figure shows the mean absolute percentage error (MAPE) for the packet dispersion and train dispersion baselines when we apply these techniques naively without having a reliable measurement framework. }
    \label{fig:unop-baselines}
\end{figure}
}
% \aqsa{problem + challenges}

}




% \vyas{strange to have two design sections. in general i dont think i learned anything useful from sec 4. what is the message of this section. if there is no useful message nuke it or move it elsewhere? it feels to me maybe sec 4 is the "putting it together section" sat the end of design rather than an overview per se. or make it a  high level view subsection of a the design section}  

==> 5-design.tex <==
\section{Design}
\label{sec:design}
% \maria{I have edited this in places that were more obvious BUT in many places this still reads like we are still working on it. This section should be more about solutions and less about challenges.}
In this section, we explain how we adapted the dispersion-based estimation to the \NFCR context. We first show analytically the connection between dispersion and NF capacity. Next, we explain how \sys process dispersion measurements to estimate the true \NF capacity; how \sys generalizes to one-sided and how it can be parameterized using the probe length.
%about the design and explaining our  process in answering them.



\subsection{Dispersion-based Strategy to \NFCR} \label{sec:dispersion}
\begin{figure}[t!]
    \centering
    \includegraphics[width=0.9\columnwidth]{fig/disp.png}
    \vspace{-0.1cm}
    \caption{\small In the two-sided threat model, the time difference between consecutive packets increases as packets exit from the \NF revealing \NF's processing time, thus its capacity. }
    \label{fig:disp}
    \vspace{-0.4cm}
\end{figure}
In this subsection, we explain how we can adapt dispersion-based bandwidth estimation approaches for \NFCR. 
Dispersion-based techniques seek to estimate the bandwidth of a bottleneck link by sending a probe of two (i.e., a pair) or more (i.e., a  train) packets back to back and measuring their spacing at the receiver. 
To see the intuition, consider the  case of a packet pair.
Assuming that the link capacity of the bottleneck link is lower than the packets' inter-arrival rate, the second packet of a packet pair will be queued, waiting for the transmission of the first one. 
The time difference between the arrival of the two packers in their destination is called {\em dispersion \disp}  and gives the transmission time $t_{tr}$ on the bottleneck link.
We can then calculate the bottleneck link capacity $C_l$ for a packet of size $S$ as follows:
%\begin{align}
  $C_l  =  S / t_{tr} = S / \delta$.  %\nonumber
%\end{align}

This basic idea assumes that processing delays on path are negligible compared to link transmission delays.
Yet, if the pair traverses an \NF the measured dispersion depends on the \NF's processing $t_p$ time, which is typically higher than transmission time since it does more than forwarding.
Hence, to adopt dispersion based bandwidth estimation for \NFCR where the packet also traverses an \NF, the dispersion is:
\begin{align}
    \delta = \max (t_{tr}, t_p) = \max (S/C_l,1/\cp)
\end{align}
Thus, if we assume that the \NF's processing time $t_p$ is larger than the transmission time $t_{tr}$ then measured dispersion corresponds to the former.
As an illustration, in  Fig.~\ref{fig:disp} the sender forwards back-to-back packets, they will be queued at the 
\NF. For each  $p_i$, the next packet  $p_{i+1}$ will only be processed  after the \NF is done processing  $p_i$ (as the \NF is single-threaded). In other words, packets are dispersed by the time it takes to process a packet at the \NF. Hence, the amount of dispersion between packets \disp at the receiver gives the processing time $t_p$ of the \NF. 
From this dispersion \disp between packets, the processing capacity \cp of the \NF can be estimated as we discuss next. 


%\begin{tcolorbox}[colback=grey!5!white,colframe=black!75!black,boxrule=0.75pt,boxsep=-0.2mm]
%\textbf{Insight} 
% Due to the lower network footprint, dispersion-based techniques are more promising.
%\sys uses dispersion based techniques to reduce the attacker's footprint.
%\end{tcolorbox}
% \begin{align}
%      \label{eq:tpp}
% \end{align} 




% For \NF capacity estimation, when we send packets back to back from sender to the node with deployed \NF sh shown in Figure~\ref{fig:disp}, the \NF processes the first packet and the second packet is queued after the first. This queuing time is equal to the packet processing time at the \NF. Hence, the packets are dispersed by the time it takes to process a packet at the \NF. Hence, the amount of dispersion between packets $\delta$ at the receiver gives the processing time $t_p$ of the \NF, from which we can calculate the capacity $C_p$ of the \NF. 

 %\ie while the \NF will be processing the first packet $p_1$ the following packets $p_2, .. ,p_\trainsize$ will form a queue behind it.

%Thus, unless these packets wait in other queues before they reach their destination each packet $p_{i+1}$ will arrive $t_p$ time after the $p_{i}$.
 % of the \NF. 

%To summarize, an attacker can use a dispersion-based technique for \NFCR under two assumptions:
%First, the link capacity of the path is greater than the processing capacity of the \NF.
%Second, the packets are sent back-to-back, which means the maximum duration between packets when they leave the sender should be less than the processing time of the \NF.


% Note that we can send more than two packet, making a packet trains which can also be used~\cite{prasad2003bandwidth}. 


%Having explained why we \sys uses dispersion, \ie measures the timing difference between received packets. 
% The next natural question is related to the choice for the train length. On the one hand, a small train will be less likely to trigger  the full \NF capacity as the observed capacity depends on the load. On the other hand, a small train is more likely to be below the budget.
 
 %On the other hand, a small train will be well within the packet budget \ie will make the attack harder to detect.


%\vyas{this feels like background on dispersion not NF specific stuff? can we better highlight what is background and what is nfcr specific} 
% \subsubsection{Train Size} 



\remove{
\begin{itemize}
    \item Goal: We want to see the maximum frequency
    \item Decision 1: We choose to send budget packets. Why? to see all possible transitions ( to maximise the likelihood of seeing the max frequency)
    \item Decision 2: We use step detection to identify frequency transitions. Why?  because naive approaches fail as shown below. 
    Naive approach No. 1: take min, sensitive to noise \\
    Naive approach No. 2: take tail, won't work if FS rolls back to lower frequency \\
    Our Approach: do step detection and then pick the window with the min disp
    \item Decision 3: We use binary segmentation for step detection. Why? Because it is less sensitive to noise. \\
\end{itemize}}

%Having explained the use of dispersion for inferring accuracy we need to make two decisions 
%the former affects how many dispersion values we will have available, while the latter the  decides how each measured dispersion will affect our end result.




\input{5b-estimation}





%\myitem{} to maximize the likelihood of triggering the frequency transition to the maximum frequency, we send packet trains of size equal to our budget \budget as sending wrong train length may not reveal the maximum frequency.




% different NFs show transitions in different locations~\ref{fig:fs-diff-nf}

% Motivate that sending longer trains helps.

% Motivate that there is absence of a trend b/c 1) same nf may have different behavior in the same node,



%\subsection{Estimation Technique}

% After sending the packet train of \budget packets, we collect dispersion of packets at the receiver. 
% For every train of size \trainsize, we calculate $\trainsize-1$ dispersion values ($D = \delta_1..\delta_\trainsize$). 
% Figure~\ref{fig:fs-ex}, shows the dispersion values we collect over the life of a train. 
% We observe that when the frequency transition happens we also see a shift in the dispersion value. 
% For inferring the capacity of the \NF we want to pick a single or a function of some of the measured dispersion values that correspond to the time when the \NF was operating at its maximum capacity. We now discuss our choice of the estimation technique below.
% \maria{@aqsa can you pick above or bellow?}


% Moreover, we found that   
% Another factor to keep in mind while choosing a step detection  algorithm is its sensitivity to noisy data. In the presence of congestion or noise from the measurement infrastructure


%\vyas{Can we add a quick putting the pieces together para or potentially figure here for this section?} 

% \mypara{Putting it all together}
% Next, we put all the pieces of the probing strategy together.  
% Consider an attacker who aims to DDoS an enterprise network. To calculate the resources that she needs, the attacker uses \sys to estimate the capacity of the firewall that the enterprise deploys at its edge. The attacker is willing to send only up to $1000$ packets ($B=1000$) to prevent the target network from detecting her attack and upgrading her infrastructure. The attacker has infected a host in the target network (two-sided threat model).  The attacker sends $1000$ in a single train of packets. Upon reception, the infected host captures those $1000$ packets, stores their timestamps and calculates the inter-arrival times between these packets (dispersion). Following \sys, the attacker applies \stepDetectionAlgo to detect the transitions (steps) in the series of computed dispersion values and calculates the mean dispersion of each step. 
% Finally, the attacker uses the minimum of the mean dispersion values to calculate the firewall's capacity.




==> 5b-estimation.tex <==
\subsection{Estimation Approach for \NFCR} \label{sec:estimation}
% \vyas{this is a vague heading. maybe say extending link estimation for nf capacity estimation? } 


%After we have chosen a probing technique, we need to decide how to estimate the capacity from the measured dispersion values. 
Unlike link bandwidth estimation, estimating the processing capacity of an \NF using dispersion requires considering additional factors. As we hint in \S\ref{sec:challenges}, these factors include: \emph{(i)} DVFS at \NF;  \emph{(ii)}  multi-threading at \NF;  \emph{(iii)}  batching at receiver. 
After defining the problem, we elaborate on how each of these factors affects the dispersion values we measure. 
Next, we explain why applying seemingly natural calculations to the measured dispersion values would not yield a correct capacity estimation.
Finally, we describe how we analyze dispersion measurements to estimate capacity.


\mypara{Problem}
After sending a packet train of \trainsize packets, we measure the dispersion of the received packets. For every train of size \trainsize, we calculate $\trainsize-1$ dispersion values ($D = \delta_1..\delta_{\trainsize-1}$). To estimate We want to compute a dispersion value that corresponds to the time when the \NF was operating at its maximum capacity. We call this dispersion value as the desired dispersion $\disp^*$ which is a function $F$ of all the measured dispersion values $D$. 



\myitem{Challenge 1: Because of DVFS, not all dispersion values correspond to the true capacity.} 
% Dynamic voltage and frequency scaling (DVFS) is a popular power management technique that allows the frequency of a CPU to be adjusted to save power and reduce heat~\cite{DVFS}, deployed by many popular CPUs  (e.g.,~\cite{SpeedStep,IntelTurboBoost}). 
Consider an \NF that runs on a CPU configured with DVFS. The CPU will operate at a lower frequency under lighter load, transitioning to a higher frequency under heavier load driven by the OS or kernel.
In the context of \NFCR, DVFS can  cause the observed rate at which packets are processed to change as  a CPU might undergo multiple transitions in frequency before reaching its maximum frequency. As a result, the measured dispersion values do not all correspond to the true capacity. For example, Fig.~\ref{fig:fs2-ex} shows the dispersion values that will actually be observed if DVFS is enabled at the \NF. The dispersion values go through multiple transitions. 


\myitem{Challenge 2: Multi-threading and batching of packets introduce spikes in dispersion values.}
As a result of multi-threading at \NF or batching at receiver, there can be spikes in the dispersion graph as shown in Figure~\ref{fig:batch-spikes}. %Hence, the estimation a;algorithm should be robust against such spikes.
%Many popular CPUs use DVFS; e.g.,  Intel's  SpeedStep technology~\cite{SpeedStep} and TurboBoost~\cite{IntelTurboBoost} and AMD implements Cool'n'Quiet technology and PowerNow technology~\cite{}. 

\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{0.49\columnwidth}
    \small
    \centering
    \includegraphics[width=\columnwidth]{fig/disp-steps.png}
    \caption{\label{fig:fs2-ex}}
    \end{subfigure}
    \begin{subfigure}[b]{0.49\columnwidth}
    \small
    \centering
    \includegraphics[width=\columnwidth]{fig/batch-spikes.png}
    \caption{\label{fig:batch-spikes}}
    \end{subfigure}
    \caption{\small (a) Assuming that the  last step corresponds  to maximum frequency is incorrect due to the potential under-clocking. (b) Batching can cause spikes in the dispersion signature. Hence, choosing a probe length larger than the batch interval is important. 
    % (c) The number of transitions observed for three real \NFs on the same deployment vary. 
    } 
    %Moreover, within an \NF on the same deployment, the number of transitions also vary.}
\end{figure}




\mypara{Strawman solutions}
A straightforward approach for $F$ would be to choose the minimum dispersion value. 
In this case $F(D) =min (\ithdisp{1},\ithdisp{2},...,\ithdisp{\trainsize})$ and the capacity \cp is given by $\cp = 1/\min (\ithdisp{1},\ithdisp{2},...,\ithdisp{\trainsize})$.
Unfortunately, this natural estimate could lead to inaccurate results. 
The minimum dispersion could represent a moment of (self-induced) congestion which would cause two packets to wait into the same queue effectively modifying their dispersion. Moreover, presence of batching and multi-threading will also distort this value.   

An alternative approach is to calculate the mean or median dispersion value across the last $N$ packets in the train, since these packets are more likely to have observed the maximum frequency, if the train itself has triggered it.
In this case, $F(D) =mean (\ithdisp{\trainsize-N},\ithdisp{\trainsize-N+1},...,\ithdisp{\trainsize})$ and \cp will be $\cp = 1/mean (\ithdisp{\trainsize-N},\ithdisp{\trainsize-N+1},...,\ithdisp{\trainsize})$.


Finally, one could chose the configuration of $N$ by finding the last step in the dispersion values using a step detection algorithm. This approach implicitly assumes that CPU frequency transitions from low to high and then remains there until the load subsides. However, we observed that in certain cases, frequency may transition back to a low frequency as shown in Fig.~\ref{fig:fs2-ex}. 


\myitem{\sys uses step detection to find the dispersion values corresponding to the maximum frequency.} 
To avoid the shortcomings of previous methods, \sys first performs step detection~\cite{truong2020selective} on the sequence of dispersion values $D=\ithdisp{1},\ithdisp{2},...,\ithdisp{\trainsize}$. Second, it divides D in to a set of segments $S$ at the detected steps.
Third, for each segment $\disp_{i\rightarrow{j}}\in S$ from \ithdisp{i} to \ithdisp{j}, it computes the mean dispersion value of the segment.  We choose mean dispersion because it generalizes to the case of batching and multi-threading. After that, \sys picks the minimum mean dispersion values as $\disp^*$. Given segments $\disp_{i \rightarrow j} \in S$, we calculate $\disp^*$ as: 
\begin{align}
    \delta^* = \min_{\ithdisp{i\rightarrow j} \in S} \dfrac{\sum_{n=i}^j(\ithdisp{n}) }{j-i+1}
\end{align}
For step-detection, we consider algorithms which do not require number of steps as input becuase the \NF may transition to many steps which will vary across deployments. Hence, we consider a different class of step detection algorithms~\cite{truong2020selective} which use penalty functions to separate noise from steps. Among these algorithms, we choose \stepDetectionAlgo~\cite{bai1997estimating} as it is widely used~\cite{chen2012parametric,fryzlewicz2014wild}.
We use the Gaussian Kernel~\cite{garreau2018consistent} as our cost function to measure variations in the data as it empirically works well. We use linear penalty~\cite{truong2020selective} for step detection based on empirical observations. 





% Many classical signal processing algorithms for step detection require prior knowledge of the number of steps~\cite{lavielle1998optimal}. 
%  However, predicting the number of transitions is challenging.
% %To illustrate the variance, 
% Figure~\ref{fig:freq-transitions} shows that the number of transitions for three separate \NFs on the same server varies across runs and across \NFs, even in the same deployment.  Thus, such approaches do not work. 


%Giving an inaccurate number of transitions to parametric step detection algorithms may miss-classify noise as transitions or miss the most important ones, effectively reducing accuracy. 

% To avoid these shortcomings, 

%bserved that it detects the steps accurately for our problem.
% \maria{@aqsa please make this clear}


% \begin{tcolorbox}[colback=grey!5!white,colframe=black!75!black,boxrule=0.75pt,boxsep=-0.2mm]
% \textbf{Insight} 
% \sys uses \stepDetectionAlgo for step detection, which does not require the total number of transitions to be known apriori.
% % \sys selects the minimum of the step dispersion values  to calculate \cp.
% \end{tcolorbox}

==> 5c-one-sided.tex <==
\subsection{\sys with One-sided Control}
\label{sec:onesided}


\sys, as we have described it so far, relies on the timestamped packets that the receiver reports. 
In this subsection, we explain how \sys can be extended to 
the one-sided threat model.
% \myitem{Q6: Who can act as a receiver in the one-sided control model?}

%Reiterating through the bandwidth estimating literature does not make our problem much easier. 
While some prior works wave the requirement of a receiver that is controlled, they are not applicable for \NFCR. For instance, Saroiu et al.~\cite{saroiu2002sprobe} send TCP SYN requests aiming at triggering a TCP RST. An alternative approach from Carter et al.~\cite{carter1996measuring} sends an ICMP ECHO REQUEST aiming at triggering a ICMP REPLY. In both cases, the solution relies on the use of particular packet types which trigger protocol-specific behavior, that might not trigger any processing from the \NF. 


\name exploits the error messages, namely \emph{ICMP time exceeded} sent as error messages from routers to hosts upon receiving an IP packet that has no time to reach its destination. 
Concretely, each IP packet carries a Time To Live (TTL) value in its header. As routers in the Internet path forward an IP packet, they decrement this value by one. If the TTL reaches zero (expires) before the packet reaches its destination, an \emph{ICMP time exceeded} message is sent by the last router that decremented it to the sender.  To trigger this behavior, the attacker: \emph{(i)} sends packets towards a destination IP that is within the IP address space allocated to the targeted network;\footnote{IP address space allocation is public information.} and \emph{(ii)}
sets the TTL of the probing packets such that the TTL expires after the packet is processed by the \NF but before the packet reaches its destination. The attacker can discover the appropriate TTL by using traceroute~\cite{TracerouteLinuxMan}.\footnote{For example, the attacker can target the last router in the path that replies to traceroute.} Traceroute is a standard measurement tool that relies on the TTL expiration mechanism and allows the sender to observe the path (the series of routers) that a packet takes to a destination. 
Importantly, TTL is part of a standard IP header and hence it generalizes to various packet types. 

%Concretely, \sys sends probes to the \NF with a certain TTL value, on expiry of these probes at the router, the router generates ICMP TTL exceeded packets. These packets are then received by the attacker who measures the dispersion from these packets. 


\begin{figure}[t!]
    \centering
    \includegraphics[width=0.9\columnwidth]{fig/router-processing.pdf}
    \caption{\small 
    One-sided threat model: While a router can be used to echo the packets back to the receiver (triggering ICMP TTL time exceeded), its processing rate may change the spacing across packets (dispersion), effectively ruining the signature.
   % The figure shows that in one sided control, when the TTL of packets expire at the router, the router may take longer time than the \NF to process the ICMP TTL Exceeded reply, thus interfering with the dispersion signature from the \NF.
    }
    \label{fig:router-processing}
\end{figure}


While promising, relying on \emph{ICMP time exceeded} to calculate \NF dispersion is challenging. In fact, the use of ICMP replies has known limitations which are well studied in the context of  traceroute~\cite{detal2013revealing,gunes2008resolving}.
We focus on three factors that are particularly impactful in our context, as they obfuscate the dispersion signals. These are related to the router processing time, contention at the router or potential rate-limiting of ICMP traffic:

\begin{packedenumerate}

\item{\em  The router processing time might overwrite the \NF dispersion.}
In this case, the observed dispersion would correspond to the router's processing time \ie not the \NF's processing time.
We illustrate this issue in Figure~\ref{fig:router-processing}.
This is not a problem in the case of two-sided in which routers only forward the probing packets (instead of dropping them and generating a new packet).

\item{\em The router in which the TTL expires might be congested with regular traffic, thus adding random delays to ICMP replies}. 
In such cases, routers prioritize regular packet forwarding from control tasks which are often best effort. The random delays added to the ICMP packets will make their dispersion useless for the attacker.

\item{\em ICMP ratelimiting may cause the routers to not respond at all.}
Finally, an operator might rate-limit the ICMP traffic~\cite{ICMPRatelimiting} for performance or security reasons. For example, in our experiments, we tried three routers in the university network and found that two of them rate-limited packets at five packets per second as also observed by Ravaioli~\etal~\cite{ravaioli2015characterizing} %characterized ICMP rate 
who foun that 60\% of the routers in the Internet implemented ICMP TTL Exceeded rate limiting.

\end{packedenumerate}





% \begin{tcolorbox}[colback=grey!5!white,colframe=black!75!black,boxrule=0.75pt,boxsep=-0.2mm]
% \textbf{Insight} 
% Under the one-sided threat model, \sys triggers an ICMP TTL Time Exceeded error to compensate for the lack of a attacker-controlled receiver. While promising relying on this error message to calculate dispersion is challenging.
% \end{tcolorbox}


% \newpage
% \myitem{Q7: How can we make ICMP errors (ICMP TTL Time Exceeded) a reliable source of dispersion?}

\myitem{\sys configures only a subset of the probing packets that are spaced in time to trigger ICMP replies. 
}


To effectively addresse the aforementioned limitations, we use two insights \sys configures only a subset of the probing packets that are strategically spaced in time to trigger an ICMP TTL Time Exceeded error from a router. This alleviates the effect of ICMP rate-limiting and the processing time of the router. 


First, while \sys needs to send large trains to trigger frequency scaling, \sys only needs the dispersion from a small number of packets to estimate \cp.
Second, to measure dispersion, \sys does not need the arrival times of consecutive packets, instead \sys can calculate the mean dispersion $\Bar{\disp}$ between two packets $p_i$ and $p_j$, which arrive at the receiver at $t_i$ and $t_j$ by $\disp = (t_j - t_i) / (j-i)$




% This means that: 1) Rate-limiting should not harm us as long as we receive a small number of packets having dispersion which corresponds to the maximum frequency.
% 2) To avoid router-processing times, we do not collect dispersion from consecutive packets. Say our router of interest has processing time f$t_ICMP$ or ICMP replies. Moreover, the \NF has processing time $t_p$. Now, we want to space packets such that when the packet k arrives at the router, the packet j has already left.

Next, we explain how we use these insights to mitigate the effects of rate-limiting, router processing times, and router load.
Consider that the attacker sends a packet train of length \trainsize at time $\tau^{send}$. The attacker sets the TTL of packet $p_i$ and some other non-consecutive packet $p_j$ to expire at some router $r$. The packets arrive at the \NF, which takes time $t_p$ to process each packet. The first packet $p_1$ sees no queuing delay at the \NF. The second packet is queued for time $t_p$ and packet $p_i$ is queued for time $(i-1)t_p$ because $i-1$ packets will be processed before the packet $p_i$. Then, the packet $p_i$ arrives at the router, which will see that $p_i$ has expired TTL, and it will generate an ICMP TTL time exceeded with processing delay $t_r$. Then, let $\tau^r_i$ be the time the reply for packet $p_i$ arrives at the sender, and  $\tau^r_j$ be the time the reply for packet $p_j$ arrives at the sender. 

If $d_i$ is the total delay when packet $p_i$ left the sender and its ICMP Reply arrived at the sender, then $\tau^r_i$ is:
\begin{align}
    \tau^r_i =& \tau^{send} + d_i \label{eq:di}\\
     \text{where }d_i =& t_p + t_r + (i-1)t_p + c \nonumber
\end{align}
$c$ is for the constant transmission and propagation delay; $t_p$ is the processing delay experienced by the packet $p_i$ at the \NF; $t_r$ is the router processing delay in generating an ICMP reply; $(i-1)t_p$ is the queuing delay experienced by the packet.
We choose packet $p_j$ such that when it arrives at the router, packet $p_i$ has already been processed. This ensures that packet $p_j$ does not see any queuing at the router. Then for packet $p_j$, $\tau^r_j$ is given by:
\begin{align}
    \tau^r_j =& \tau^{send} + d_j  \label{eq:dj}\\
    \text{where } d_j = & t_p + t_r + (j-1)t_p + c \nonumber
\end{align}
At the sender, we can calculate the dispersion as follows:
\begin{align}
    \disp =  \tau^r_j -  \tau^r_i \label{eq:od}
\end{align}
% Substituting Equation~\ref{eq:tri} and Equation~\ref{eq:trj} into Equation~\ref{eq:od}, we get:
% \begin{align}
%      \disp = &\tau^{send} + d_j  - \tau^{send} + d_i \nonumber\\
%      \disp = &d_j - d_i \label{eq:od2}
% \end{align}
Substituting Equation~\ref{eq:di} and Equation~\ref{eq:dj} in \ref{eq:od}, we get:
\begin{align}
    \disp =&\tau^{send} + t_p + t_r + (j-1)t_p + c  \nonumber \\ & - \tau^{send} - t_p - t_r - (i-1)t_p - c \nonumber \\
    \disp = &(j-i)t_p \label{eq:fod}
\end{align}
From Equation~\ref{eq:fod}, the processing capacity \cp can be estimated as follows:
\begin{align}
    \cp = 1/t_p = (j-i)/\disp
\end{align}
%The one-sided attacker model assumes that we know the IP address of at least one public server inside the private enterprise.
%Hence, we can get knowledge about the routers in the path by running a Traceroute~\cite{}. 
%We also want the router after the \NF, so that when packets expire at the router, they already contain the dispersion signature from the \NF. This can be done by picking routers closer to the public server, and also by looking at the AS of the routers.
% 
% \myitem{Q8: How to choose the correct gap between packets to set the TTL?}
Having explained why we do not need to trigger an ICMP error in every packet of our probe, the next natural question is how to choose these packets. To decide that, we need to look at our constraints. We want to space the packets such that when packet $p_j$ arrives at the router, packet $p_i$ has already been processed. This requires an estimation of an \emph{upper-bound} of router processing time. We can estimate processing time by sending packet pairs with the correct TTL. 
The spacing of the replies will give the router processing time. For example, in our experiments, we found that the router took 55us to process and generate ICMP replies. 

Once we have an estimation of the router processing time, we can choose the packets such that when they arrive at the router, they are at least $t_r$ apart. For example, for a router processing time of 100us, we can set the TTL after every 100 packets, assuming our send rate is 1Mpps. Concretely, for a router processing time of $t_r$, and the maximum capacity $C_{max}$ that the attacker can send, we can set the TTL after a gap of $g_{TTL}$ packets where $g_{TTL}$ is chosen such that $g_{TTL} > t_r \times C_{max}$, $t_r \times C_{max}$ gives the num,ber of packets that arrive at the router in time $t_r$. 
Observe that the \NF processes packets before they arrive at the router. Thus, the actual duration between the packets will be much greater than $t_r$. 
For example, consider that we have an \NF, which processes each packet in 5us, and a router takes 100us to generate an ICMP reply. If the sender sets the TTL of every 100th packet, then if the first packet arrives at the router at time t, the 101st packet will arrive at $((5us) + (100)(5us))\times t$, which is much greater than 100us. 
Importantly, the estimation of the processing in the router need not be extremely accurate. In fact, we only need to make sure that the packets are spaced out more than the processing time.

%


%

\remove{
\name exploits the \emph{ICMP time exceeded} messages sent as error messages from routers to hosts upon receiving a packet that has no time to reach its destination. Such a solution is not trivial, though, due to the processing time at the router and the rate-limiting of such packets as shown in Figure~\ref{fig:rate-limiting}. For example, in our experiments, we tried three routers in the university network and found that two of them rate limited packets at 5 packets per second. This is in sync with the extended study of Ravaioli\etal~\cite{ravaioli2015characterizing} %characterized ICMP rate 
who found that 60\% of the routers implemented ICMP TTL Exceeded rate limiting. 
}

% \mypara{Putting it together:}
% We use the same example as we used at the end of \S~\ref{sec:design}, but now we assume that the attacker has no colluding host inside the enterprise network. Like the two-sided scenario, an attacker sends a train of $1000$ packets, but this time to a destination IP among the IPs assigned to the enterprise. The attacker uses traceroute to determine that the path from herself to the destination is eight hops. For every $300$ packets that the attacker sends, she sets one packet with TTL=7 (total of three packets). These three packets trigger an ICMP TTL exceeded from a router one hop away from the destination IP, which arrive at timestamps t1, t2, t3 respectively. The attacker estimates 
% $C_p = min(\frac{300}{t2-t1}, \frac{300}{t3-t2})$.







==> 5d-probing-length.tex <==
\subsection{Probe Length}\label{sec:length}

% \vyas{isnth this logically before the one sided estimator?} 

In this subsection, we explain how many packets the attacker needs to send (probe length) to have an accurate estimation. Figure~\ref{fig:decision-tree} summarizes our insights into the various factors that play a role in this decision.
% \myitem{Q2: How many packets should we send per probe/train?}
The ideal probe length for the attacker, \ie the minimum number of packets for a good estimation depends on all the factors we have mentioned so far including \NF's deployment, the receiver's existence, or hardware configuration.

%\myitem{In one-sided \sys, the probe length depends on the TTL gap.}
Starting from the bottommost path in Figure\ref{fig:decision-tree}:
If the attacker is one-sided, meaning they only control the senders and rely on a router for receiving some form of reply, she would need to send $c_1  \times g_{TTL}$ where  $g_{TTL}$ is the gap between packets for which the attacker sets the TTL, and $c_1$ a constant which determines the number of TTL Exceeded packets the attacker will receive.  
Remember that in the one-sided case, to deal with routers with longer ICMP router processing times, and with ICMP rate-limiting, \sys spaces out the packets with the correct TTL. This gap determines the length of the probe. In our experiments, $30\times g_{TTL}$, with $g_{TTL}$ of 100 packets (total of 3000 packets ) yields accurate capacity estimations.  In the presence of DVFS, the attacker will again need to send packets in the order of thousands to first trigger DVFS.


If the attacker is two-sided and the \NF does not use DVFS (topmost branch), then the probe length will depend on the number of threads in the \NF or/and the batch interval in case of packet batching. First, to capture the affect of multi-threading, the attacker will need to send packets $c \times k$ packets at the \NF with $k$ threads, where $c$ is some constant. Intuitively, the value of $c$ is proportional to the number of threads. 
Second, to handle the noise introduced by batching, attacker will need to send packets such that the total arrival time of packets at the receiver is larger than the batch interval. 
Batching is usually done in microseconds with typical value being in hundreds~\cite{dovrolis2004packet, training_2024}. Hence, in this branch of the decision tree, a few hundred packets will give a good estimate, assuming that the number of threads is also in hundreds.

If the attacker is two-sided and the \NF uses DVFS, the packets needed to trigger DVFS will be in thousands and hence the number of threads and batching will not play a role in determining the probe length. Similarly, in the one-sided case, the number of packets typically needed would be in thousands. Hence, multi-threading and batching may also not play a role there.

\remove{
\myitem{DVFS requires a probe length in the order of thousands of packets to cause a transition to the maximum frequency.}
First, DVFS can significantly affect the accuracy of \sys.  Consider an \NF that runs on a CPU configured with DVFS. In effect, the CPU will operate at a lower frequency under lighter loads, transitioning to a higher frequency under heavier load driven by the OS or kernel. The change in frequency also changes the processing rate of the \NF and thus the processing time per packet. Thus, sending a short packet train will not reveal the maximum capacity \cp of the \NF as shown in Figure~\ref{fig:fs-ex}.
As an example, Figure~\ref{fig:fs-diff-nf} shows the fraction of probes that triggered a frequency transition as a function of the train size. For instance, 59\% of the probes triggered a transition after having sent $1000$ packets (orange line). In effect, if the attacker sent $1000$ packets, she would have 59\% chance of observing the true capacity. We also observe that there can be multiple transitions. Concretely, we observe that almost 100\% of our probes of $300$ packets trigger a transition (blue line). This is critical as it means that simply gradually increasing the train size to trigger  a transition will fail. Indeed, such an attacker will have no way of knowing whether the CPU would undergo more transitions if she continued increasing the train size. 

Predicting the behavior of frequency scaling is hard because they are controlled at multiple levels, in the BIOS (\eg Dell's DBPM~\cite{beckett2012bios}) as well as by the OS~\cite{DVFS}. Moreover, different deployments may differ in their configurations.  Thus, we argue our best strategy is to send as many packets as possible to maximize the load to the CPU, effectively triggering the highest frequency to get a realistic view of the \NF capacity.
}

\begin{figure}[t!]
    \centering
    \includegraphics[width=0.9\columnwidth]{fig/d3.png}
    \caption{\small Probing an \NF to estimate its capacity is challenging because of factors such as if the attacker controls nodes on both sides of the \NF or not, if there is DVFS enabled in the \NF deployment, batching of packets etc.}
    \label{fig:decision-tree}
    \vspace{-0.3cm}
\end{figure} 
\begin{figure}[t]
    \centering
  \includegraphics[width=0.75\columnwidth]{fig/fs-transitions.png}
      \caption{\small \label{fig:fs-diff-nf} Poorly-selected train size may not trigger a transition to the maximum frequency; e.g., a train of 1000 packets has only 59\% chances of observing the \emph{maximum} frequency and 100\% chances of observing the first transition to a higher frequency.
      }
\end{figure}
% \begin{tcolorbox}[colback=grey!5!white,colframe=black!75!black,boxrule=0.75pt,boxsep=-0.2mm]
% \textbf{Insight} To improve the chance of triggering a transition to the maximum CPU frequency given a budget, \sys sends a budget-length train.
% \end{tcolorbox}

\remove{
\myitem{Multi-threading requires a probe length in the order of the number of threads.}
Second, presence of multi-threading at the \NF will also affect \sys's accuracy. \sys will not accurately measure the capacity if it does not trigger all the threads. Hence, the attacker will need to send at least as many packets as the number of threads.  
% Actually, if the attacker wants the error to be less than some $\epsilon$, then the attacker needs to send a probe longer than:


\myitem{Packet batching requires a probe length longer than the batch interval.}
Third, presence of batching at the receiver introduces error as we show in the Evaluation~\ref{sec:evaluation}. This happens because all the packets which are batched together will show the same timestamp at the receiver. To handle this, the attacker has two choices. The attacker can either turn off packet batching at the receiver if the attacker has access to hardware at the receiver. (This may not be the case if \eg the attacker has a VM at the receiver). If batching cannot be turned off, then the attacker will have to send at least as many packets as the batch interval. 
}
% In fact, if the attacker wants the error to be less than some $\epsilon$, then the attacker needs to send a probe longer than:
%Second, the function will use to select a single dispersion across all measured dispersion values.
%The former question affects how many dispersion values we will have available. 
%The latter question decides how each measured dispersion will affect our end result.


%To justify this decision we first provide the required background about frequency scaling by the CPU, which is the key factor for the difference in the observed capacity over time. 
%IF 
%$$\subsubsection{Dynamic voltage and %$frequency scaling} 
%\label{sssub:dvfs}
% Dynamic voltage and frequency scaling (DVFS) is a popular power management technique that allows the frequency of a CPU to be adjusted to save power and reduce heat~\cite{DVFS}, deployed by many popular CPUs  (e.g.,~\cite{SpeedStep,IntelTurboBoost}). 
%DVFS can appear in the form of CPU throttling, \ie under-clocking the CPU, or in the form of CPU boosting, \ie overclocking the CPU. 

%In the context of \NFCR, DVFS can  cause the observed rate at which packets are processed to change as  a CPU might undergo multiple transitions in frequency before reaching its maximum frequency. 
%Many popular CPUs use DVFS; e.g.,  Intel's  SpeedStep technology~\cite{SpeedStep} and TurboBoost~\cite{IntelTurboBoost} and AMD implements Cool'n'Quiet technology and PowerNow technology~\cite{}. 





%Having an intuition of the potential effect of DVFS, 

% We empirically study the number of packets that we need to send to trigger frequency transitions in various CPUs




% \vyas{in general i would be lost after reading sec 5. i dont see how these things fit together. some scaffolding text/ideas at the end on how all of these come together maybe using the decision tree will help the reader}

% \vyas{also as a writing style nit -- there is just WAY too much bold in sec 5 and through the paper. so i dont actually know what is worth focusing on :) -- please use bold etc sparingly} 

==> 6-eval.tex <==
\section{Evaluation}\label{sec:evaluation}

We evaluate the accuracy and the stealthiness of \sys in two representative configurations, namely \syslarge and  \syslite, which send \dvfslength and 100 packets, respectively in controlled and Internet experiments.
We find that \syslarge is up to \syslargedelta more accurately than a baseline sending the same number of packets per probe.
\syslite is accurate only on a subset of the NF deployments but is more stealthy. 
\syslite is up to \syslitedelta more accurate in controlled experiments compared to the equivalent baselines sending the same number of packets. 
Importantly, we find that \syslite can accurately estimate the capacity of a commercial \NF in AWS  within \sysliteaws of error.
We also evaluate the impact of each individual optimization in \sys and find that step-detection and an optimized measurement infrastructure are crucial to \sys's accuracy.

\begin{figure}[t!]
    \centering
% \begin{subfigure}[b]{0.32\textwidth}
%   \centering
%     \includegraphics[width=0.9\columnwidth]{fig/internet.pdf}
% %     \caption{\label{fig:internet-setup}}
% \end{subfigure}    
% \begin{subfigure}[b]{0.32\textwidth}
   \centering
    \includegraphics[width=0.9\columnwidth]{fig/setup.png}
% \end{subfigure}


\caption{\label{fig:internet-setup} Our Internet setup forwards packets through the Internet after they have been processed by the \NF. This is the worst-case scenario for the attacker (and \sys) as the Internet noise can affect the dispersion. 
In the one-sided experiments, we send probes to the Clemson node but they expire on path, causing ICMP replies to the sender(shown in dotted).}
\Description[Internet Setup]{Our Internet setup forwards packets through the Internet after they have been processed by the \NF. This is the worst-case scenario for the attacker (and \sys) as the Internet noise can affect the dispersion signature of \NF. In the one-sided experiments, we send probes to the Clemson node but they expire on path, causing ICMP replies to the sender(shown in dotted).}
\end{figure}

\subsection{Methodology}
%\myitem{Controlled Setup:} For our controlled environment, we use three nodes in CloudLab~\cite{duplyakin2019design}, a sender, a receiver and an \NF connected such that the sender communicates to the receiver via the \NF node. All Intel Haswell EP nodes with two 10-core CPUs with 2.60 GHz frequency. \\
%\myitem{Internet Setup:}
%For the experiments in the Internet, our sender and the \NF node run in CloudLab Wisconsin, and our receiver node runs in Clemson. As we illustrate in Figure~\ref{fig:internet-setup}, the packets from the \NF to the receiver go through the Internet. We stress that this is the worst-case scenario for the attacker. Indeed, if the packets in a probe see congestion in the Internet before reaching the \NF, the random delay/noise from the Internet would not affect the \NF-induced dispersion. We run this experiment at different times of day to capture the affect of varying congestion in the Internet. The sender and the receiver use the same nodes as in the controlled environment. The receiver uses Intel Haswell E5-2683 v3 nodes with 14-core CPUs and 2.00 GHz frequency. \\
%\myitem{One-sided Setup:}
%We illustrate the setup of this experiment in Figure~\ref{fig:internet-setup}. The sender and the \NF are in the Wisconsin cluster and they send packets to a public server in the Clemson cluster. The TTL is set such that the it expires in 4 hops after being processed by the NF. 

% The receiver node uses interrupt coalescencing with an interval of 300us. 

\myitem{Probing baseline:} 
We evaluate our approach against a rate-based bandwidth-estimation technique, namely \slops in which the attacker uses binary search for \NFCR~\cite{jain2002end} between 0-500Kpps. 
The attacker sends packets to the NF at an initial probing rate (250Kpps) and uses one-way delay of received packets to see if the probe
rate (pps) caused congestion indicating that the rate was greater than the NF capacity. If so, it
adjusts the probe rate accordingly using a binary search
approach.  \slops keep probing until the difference
between minimum and maximum rate is 1000pps. To
find an increasing trend in the relative one-way delay values, we
use the technique implemented by Pathload~\cite{jain2002end}. 
Moreover, we use the same probe length for the baseline and for \sys.
% \maria{re-read the above para one-way delay is not connected with the rest}

\myitem{Estimation baselines:}
To evaluate the estimation technique used by \sys, we compare with two baseline approaches adopted from the link bandwidth estimation literature \emph{(i)} 
\myitem{\bone} which takes the mean dispersion of the entire train~\cite{dovrolis2001packet}; and \emph{(ii)} \myitem{\btwo} which takes the median dispersion~\cite{li2008wbest}. 

\myitem{Network functions:} We use five \NFs.
Both \snortrl and \surrl are realistic TCP SYN rate-limiting \NFs which we implemented in Suricata~\cite{Suricata} and Snort~\cite{SnortNetworkIntrusion} respectively.
Both \NFs track the number of SYN packets per flow and drop the SYNs of flow that have exceeded a threshold. For \snortrl and \surrl, we send SYN packets.
\surbl is a deny list containing rules provided by the emerging threats database~\cite{ProofpointEmergingThreats}. We only send UDP traffic to \surbl to trigger the rules concerning UDP traffic. We implemented \surbl in Suricata~\cite{Suricata}. 
\surblmulti and \surrlmulti are multi-threaded versions of \surbl and \surrl respectively.

\begin{table}[!t]
\small
    \centering
    \begin{tabularx}{0.9\columnwidth}{clll}
    NF  ($\mu s$) & Controlled & Internet & One-sided\\
        \hline
      \snortrl & 67500 & 21000 & 21800\\
      \surbl & 142600  & 134640 & 143420\\
      \surrl & 200880 & 193750 & 225140\\
      \surblmulti & 227720  & 224680 & 216000\\
      \surrlmulti & 336060  & 360460 & 309140\\
      \bottomrule
    \end{tabularx}
    \caption{The ground-truth processing capacity of our NFs measured in packets per second (pps) for our experimental setups. Processing capacity varies for different NFs and across deployments (\eg processors, NIC, configuration)}
    \label{tab:nf-benchmark}
\end{table}

\begin{figure*}[t!]
\small
\centering
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\columnwidth]{fig/fs-lab.pdf}
        \caption{\label{fig:nfty-large-lab}}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\columnwidth]{fig/estimations.pdf}
     \caption{\label{fig:step-detection-result}}
     \end{subfigure}
      \begin{subfigure}[b]{0.32\textwidth}
       \includegraphics[width=\columnwidth]{fig/probe-len.pdf}
       \caption{\label{fig:budget}}
      \end{subfigure}
      \vspace{-1pt}
    \caption{(a) \syslarge is up to \syslargedelta more accurate than the baseline in optimized \NF deployments for the same probes length.  (b) By applying step detection to the dispersion values, the MdAPE of \syslarge is reduced by up to \stepdetectiondelta. \maria{add to label step-detection?}  (c) As we increase the probe length, the accuracy of \sys improves.}
    \Description[\syslarge Performance]{(a) \syslarge is up to \syslargedelta more accurate than the baseline in optimized \NF deployments for the same probes length.  (b) By applying step detection to the dispersion values, the MdAPE of \syslarge is reduced by up to \stepdetectiondelta. \maria{add to label step-detection?}  (c) As we increase the probe length, the accuracy of \sys improves.}
\end{figure*}
\myitem{Ground-truth measurements:} 
To measure the ground-truth processing capacity for our \NFs, we send packets to a receiver node via each \NF using Scapy $\mathit{sendpfast}$ ~\cite{rohith2018scapy}. We do a binary search on the sending rate until we find the maximum rate that allows the input rate of the \NF node, to equal its output rate (\ie the maximum sending rate without packet drops at the \NF). 
We repeat this exercise five times and choose the median as the ground-truth.
We show our results in Table~\ref{tab:nf-benchmark}.
We measure the ground-truth capacity for each setup and \NF separately, as it can be affected by hardware and software factors (\eg processor, NIC). 
We repeat each experiment 100 times and report the Median Absolute Percentage Error (MdAPE) in the estimated processing capacity compared to the ground truth (Table~\ref{tab:nf-benchmark}). 



\begin{figure*}[t!]
\small
\centering
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\columnwidth]{fig/nfty-lite-lab.png}
        \caption{\label{fig:nfty-lite-result}}
    \end{subfigure}
    \begin{subfigure}[b]{0.33\textwidth}
        \includegraphics[width=\columnwidth]{fig/batching.pdf}
     \caption{\label{fig:batching}}
     \end{subfigure}
      \begin{subfigure}[b]{0.32\textwidth}
       \includegraphics[width=\columnwidth]{fig/internet-results.png}
       \caption{\label{fig:nfty-lite-internet-result}}
      \end{subfigure}
    \caption{(a) \syslite results in 3\% to \sysliteerrorlab error in the estimated processing capacity with the optimized measurement infrastructure. \slops-100 results in high error (up to 61\%) for faster \NFs as the sender cannot send packets faster than the \NF because of DVFS at sender. (b) When we use \syslite in an optimized measurement infrastructure, the MdAPE is reduced by up to \measurementoptdelta.  The improvement is significant for the larger batch interval (batch-300us) as compared to the smaller interval (batch-100us). (c) \syslite's error remains below \sysliteinterneterror in the internet. The spread is a bit higher than the controlled experiments for very fast \NFs due to the noise added by the Internet.  }
    \Description[\syslite Performance]{(a) \syslite results in 3\% to \sysliteerrorlab error in the estimated processing capacity with the optimized measurement infrastructure. \slops-100 results in high error (up to 61\%) for faster \NFs as the sender cannot send packets faster than the \NF because of DVFS at sender. (b) When we use \syslite in an optimized measurement infrastructure, the MdAPE is reduced by up to \measurementoptdelta.  The improvement is significant for the larger batch interval (batch-300us) as compared to the smaller interval (batch-100us). (c) \syslite's error remains below \sysliteinterneterror in the internet. The spread is a bit higher than the controlled experiments for very fast \NFs due to the noise added by the Internet.  }
\end{figure*}



\subsection{Controlled experiments} \label{sec:controlled}
We start by comparing \syslarge and \syslite to baselines in a controlled lab experiment of three nodes in CloudLab~\cite{duplyakin2019design}, a sender, a receiver, and an \NF connected such that the sender communicates to the receiver via the \NF node. All Intel Haswell EP nodes with two 10-core CPUs with 2.60 GHz frequency. 
%We give an overview of how \syslarge and \syslite perform against baselines. We focus on the two-sided model because our baseline does not work for the one-sided threat model.
%We use a controlled lab experiment to investigate how \sys design decisions contribute to its precision.  

%\myitem{Controlled setup:} We use three nodes in CloudLab~\cite{duplyakin2019design}, a sender, a receiver, and an \NF connected such that the sender communicates to the receiver via the \NF node. All Intel Haswell EP nodes with two 10-core CPUs with 2.60 GHz frequency. 



\myitem{\syslarge outperforms probing baselines by 2x-\syslargedelta while sending less packets in total.}
Figure~\ref{fig:nfty-large-lab} shows the MdAPE in the estimated capacity by \syslarge and \slops. 
\syslarge results in 2\%-\syslargeerrorlab error for the five \NFs and outperforms the baseline. The improvement is more prominent in the faster \NFs, compared to \snortrl, which is slower (see Table~\ref{tab:nf-benchmark}). 
The baseline also ends up sending 9x more packets (median in NFs) than \syslarge, due to its iterative probing. Still, the baseline's poor accuracy is due to its obliviousness to the fluctuation of  one-way delays caused by the NF's optimized deployment (\ie frequency transitions). Moreover, for multi-threaded NFs (last two bars), the baseline ends up triggering only a single thread because both the multi-threaded \NFs assign packets to threads on the basis of flow.
Importantly, both techniques use the optimized measurement infrastructure we describe in \S\ref{sec:measurements}. The baseline precision further degrades with an unoptimized measurement infrastructure, as we show later (Figure~\ref{fig:nfty-lite-result}). 

\myitem{Step-detection improves \syslarge accuracy by up to \stepdetectiondelta}
To investigate the benefit of step detection, we compare \syslarge with the estimation baselines, \bone and \btwo. We summarize our results in Figure~\ref{fig:step-detection-result}. We observe that the reduction in MdAPE is significant. For  \snortrl the improvement over the baseline is less compared to the other NFs because \snortrl changes to maximum frequency sooner than the other \NFs. In effect, \bone is closer to the one corresponding to the maximum frequency. \btwo precision degrades further for multi-threaded \NFs, because of the fluctuations in queueing delays for subsequent packets it causes.



\myitem{Longer probe lengths are critical for NFs with DVFS.} 
Figure~\ref{fig:budget} shows the effect of different probe lengths on \sys's error in the presence of DVFS. Longer trains for \sys result in low errors (MdAPE) because they always trigger the transition to the maximum frequency. In contrast, small trains never trigger the transition to maximum frequency. Thus, if the attacker were to perform \NFCR with \syslite in the presence of DVFS, she would have a high error. The frequency transitions happen sooner for slow \NFs as compared to the faster ones. Note that all \NFs show a transition at length of 500 packets.

\myitem{\syslite accurately estimates capacity within \sysliteerrorlab of error.}
Since we have shown that \syslite cannot estimate the capacity of NFs whose deployments are optimized with DVFS (Figure\ref{fig:budget}), we evaluate \syslite for simpler \NF deployments. We find that \syslite estimates the capacity of these with 2\% to \sysliteerrorlab error as shown in Figure~\ref{fig:nfty-lite-result}. 
We compare \syslite with \slops-100. For \syslite, we turn DVFS off at sender, as with small number of packets, its effect becomes significant. For the baseline, DVFS is not off at the sender.
We observe that the error and the spread for \slops-100 increase up to ~61\%. Specifically, for \slops-100 the error is huge for \NFs (\surrl to \surrlmulti) where the attacker cannot send at rates higher than the \NF processing speed. This highlights the importance of our sender-side optimizations. Hence, if an attacker were to use \slops-100 without our sender-side optimization, she would incur a huge error.



\myitem{\sys's measurement optimizations improve the accuracy of \syslite  by up to \measurementoptdelta}
In the previous experiment, we already hinted that the most impactful factor in  \syslite accuracy is the measurement infrastructure, as we discuss in \S\ref{sec:measurements}. To verify that we plot 
the overall improvements caused by our measurement optimizations in Figure~\ref{fig:batching} . For the unoptimized measurement infrastructure, DVFS is enabled at the sender, and we show two receiver configurations, one with a batch interval of 100us and the other with a batch interval of 300us. For the optimized measurement infrastructure, DVFS is disabled at the sender, and there is no packet batching. 
As shown in Figure~\ref{fig:batching}, our  measurement-infrastructure optimizations in \syslite, reduce its MdAPE by upto \measurementoptdelta. 

\myitem{\sys is less detectable than \slops while being more accurate}
To evaluate the detectability of \sys, we use the ruleset of known commercial firewalls Palo Alto Networks (PANW)~\cite{}, Juniper~\cite{}, Fortinet~\cite{}, and Snort community rules~\cite{}. We implement these rulesets in Suricata, and record if these rulesets detect \sys and \slops. Table~\ref{tab:detect} summarizes our results for TCP SYN traffic processed by \surrl, \surrlmulti, and \snortrl and UDP traffic processed by \surbl, and \surblmulti. A tick indicates that the firewall was able to detect the attack. A cross indicates that the attack is not detected. Overall, \sys is less detectable than the baseline.




\begin{table}[t!]
\small
    \centering
    \begin{tabular}{c|c|cccc}
    && PANW & Juniper & Fortinet & Snort\\
    \midrule
    %  & \multicolumn{4}{c}{TCP SYN} \\
    % \midrule
    \syslarge & \multirow{4}{*}{TCP SYN} & \redcross & \redcross & \greentick & \redcross \\
    \slops-5K & &\greentick & \greentick & \greentick & \redcross \\
    \syslite & &\redcross & \redcross & \redcross & \redcross \\
    \slops-100 && \redcross & \redcross & \redcross & \redcross  \\
    \midrule
     % & \multicolumn{4}{c}{UDP} \\
    % \midrule
    \syslarge & \multirow{4}{*}{UDP} & \redcross & \greentick & \greentick & \redcross \\
    \slops-5K &&  \greentick & \greentick & \greentick & \redcross \\
     \syslite && \redcross & \redcross & \redcross & \redcross \\
     \slops-100 &&  \redcross & \greentick & \redcross & \redcross \\
     \multicolumn{2}{c}{\redcross $=$ not detected} & \multicolumn{2}{c}{\greentick $=$ detected} \\
     
    \end{tabular}
    \caption{\sys is  less detectable than \slops while being more accurate \maria{What are the columns?}}
    \label{tab:detect}
    \vspace{-5pt}
\end{table}




\subsection{Internet-2 and One-sided Experiments}
\label{sec:internet}
So far we only evaluated \name in pristine network conditions. 
Having shown that \name  outperforms baselines by orders of magnitude, in this subsection we aim to verify whether \sys is usable in more realistic settings \eg on the Internet or in cases where the attacker only controls the sender (single-sided) and thus relies on a router. 


\myitem{Internet setup:} Our sender and the \NF node run in CloudLab Wisconsin, and our receiver node runs in Clemson. As we illustrate in Figure~\ref{fig:internet-setup}, the packets from the \NF to the receiver go through the Internet. We stress that this is the worst-case scenario for the attacker. Indeed, if the packets in a probe see congestion in the Internet before reaching the \NF, the random delay/noise from the Internet would not affect the \NF-induced dispersion. We run this experiment at different times of the day to capture the effect of varying congestion in the Internet. The sender and the receiver use the same nodes as in the controlled environment. The receiver uses Intel Haswell E5-2683 v3 nodes with 14-core CPUs and 2.00 GHz frequency. \\


\myitem{Both \syslite and \syslarge remain within \sysliteinterneterror error in the Internet.}
 We evaluate \syslite (without DVFS at the \NF) in the Internet to show that \sys can accurately estimate the capacity even in the Internet using only a small number of packets.  We summarize our results in Figure~\ref{fig:nfty-lite-internet-result}. \syslite can accurately estimate \NF's capacity within \sysliteinterneterror error. The spread in error values for faster \NFs is higher than in controlled experiments.
We also evaluate \syslarge (with DVFS at the \NF) to show that even with added noise from the Internet, shown in Figure~\ref{fig:internet-fs-results} the \syslarge's estimation using step detection works well.
\syslarge has a higher spread in MdAPE in the Internet compared to the controlled environment. However, the MdAPE in the Internet for \syslarge also remains within \syslargeinterneterror error.


\begin{figure}[t!]
    \centering
\begin{subfigure}[b]{0.49\columnwidth}
  \centering
    \includegraphics[width=\columnwidth]{fig/fs-internet-30.png}
    \caption{\label{fig:internet-fs-results}}
\end{subfigure}    
\begin{subfigure}[b]{0.49\columnwidth}
   \includegraphics[width=\columnwidth]{fig/one-sided-results-30.png}
    \caption{  \label{fig:one-sided}  }
\end{subfigure}
\caption{(a) \syslarge results in 4\% to \syslargeinterneterror MdAPE in the Internet with optimized \NF deployment (with DVFS). (b) \sys results in 4\%-\sysonesidederror MdAPE with one-sided control.  In both cases, the spread in error is a bit high for fast \NFs compared to \snortrl, \ie  the slowest \NF.}
\Description[\syslarge Performance on Internet]{(a) \syslarge results in 4\% to \syslargeinterneterror MdAPE in the Internet with optimized \NF deployment (with DVFS). The spread in error increases with faster \NFs. (b) \sys results in 4\%-\sysonesidederror MdAPE with one-sided control.  Our spread is a bit high for fast \NFs compared to \snortrl, \ie  the slowest \NF.}
\end{figure}



\myitem{One-sided setup:}
We illustrate the setup of this experiment in Figure~\ref{fig:internet-setup}. The sender and the \NF are in the Wisconsin cluster and they send packets to a public server in the Clemson cluster. The TTL is set such that it expires in 4 hops after being processed by the NF. We choose $g_{TTL}$ (\ie the gap in packets for which we set the correct TTL) to be 100 packets.


\myitem{\syslarge is usable under the one-sided threat model.} 
% \maria{shouldn't this be \syslarge?}
We summarize our results in Figure~\ref{fig:one-sided}. For the experiments with one-sided threat model, 
\syslarge's MdAPE remains around \sysonesidederror. Faster \NFs such as \surrlmulti show a higher spread as in the case of two-sided Internet experiments. 
This shows that indeed, \sys with one-sided control is feasible and can result in reasonable estimation of the processing capacity of an \NF.





\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{0.48\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{fig/aws-setup.png}
    \caption{\label{fig:aws-setup}}
\end{subfigure}
\begin{subfigure}[b]{0.48\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{fig/aws-result.png}
    \caption{\label{fig:aws}  }
\end{subfigure}
\caption{ (a) In the AWS experiments,  the sender probes the \NF from the Internet. (b) \syslite results in \sysliteaws MdAPE while probing a commercial \NF Fortinet next generation firewall~\cite{fortinet}. The spread is high because here, the receiver and the NF are VMs and may induce extra noise.}
\Description[AWS Experiments]{(a) In the AWS experiments,  the sender probes the \NF from the Internet. (b) \syslite results in \sysliteaws MdAPE while probing a commercial \NF Fortinet next generation firewall~\cite{fortinet}. The spread is high because here, the receiver and the NF are VMs and may induce extra noise.}
\end{figure}


\subsection{Internet Experiments}
Now we evaluate NFTY outside of the Internet2 setting which had packets sent only between Cloudlab machines. In these experiments, we provide an even more realistic setting for an attacker operating in a two sided model where they control both the sender and receiver.  \newline
\myitem{Internet setup:} Our sender and the NF run in Cloudlab Wisconsin, and our receiver node runs in Vultr Los-Angeles. Similar to figure 6, as the packets travel from the Cloudlab machines to the Vultr machine, they traverse the Internet. Unlike in the Internet2 experiments, the packets are no longer travelling through the isolated environment that the Cloudlab network services provide. We run these experiments with an unoptimized NF (DVFS off) and an optimized sender (DVFS off) and at different times of day to capture any variance caused by time of day. We perform these experiments with an unoptimized NF to see the viability of NFTY in the internet setting. The sender and NF use the same nodes as the previous experiments, and the receiver uses an Intel E-2288G processor with 8-core CPUs and 4.70 GHz frequency. Our experiments utilize the 2-sided method. 



\myitem{NFTY-5K remains within 8\% error in the Internet.} Figure ~\ref{fig:int-5k} shows that the MdAPE for NFTY-5k in this setting never exceeded 5\% for all \NFs. For all 100 experiments for each NF, the calculated error never exceeded 8\%. Thus, NFTY-5K achieves very low error rates even in the Internet environment such that we have DFVS disabled at the \NF.  We can also infer that, due to the closeness of the MdAPE and maximum error, that there is little spread and variance of NFTY-5K in the Internet. Thus, NFTY-5K proves itself as a reliable method where noise and delays may be prevalent.  Like our previous experiments, we also see a general trend where the faster \NFs have larger MdAPE results due to more noise in the dispersion values when the packets are sent across the Internet. \newline
\myitem{NFTY-100 results in less than 10\%  MdAPE for single-threaded NFs. } Figure~\ref{fig:int-100} indicates that NFTY-100 achieves low MdAPE values for the single-threaded \NFs: SNORT-RL, Suricata-RL, and Suricata-BL. None of these MdAPE values exceeded 6\%, demonstrating the high accuracy that NFTY-100 can achieve in the Internet setting with such a small amount of packets. Compared to the spread of the Internet2 experiments, NFTY-100 has a greater spread  (not shown in figure~\ref{fig:int-100}) due to the added noise of the Internet.  For the multi-threaded \NFs, there are two queues that packets are processed in, and so each queue processes only 50 packets each. With so few dispersion values for each queue and the noise of the Internet prevalent at the beginning of a probe, NFTY produces an inaccurate estimate. Figure ~\ref{fig:int-5k} indicates that using 5000 packets instead for NFTY produces far more accurate results that outweighs the noise of the Internet that is prevalent in the first 100 packets of the probe. \newline
\myitem{Both NFTY-100 and NFTY-5K consistently outperform SLoPS.} When comparing performance of NFTY to SLoPS, it has a smaller MdAPE for all NFs for both techniques. As seen in the results for the controlled environment and Internet2, SLoPS performs poorly for the multi-threaded \NFs. This is because the threads are assigned to based on flow, and SLoPS sends all packets to only one thread, thus predicts the processing capacity of only one queue.  Although NFTY-100 has reduced accuracy for the multi-threaded \NFs, it still outperforms SLoPS. When comparing performance for the single-threaded \NFs, NFTY-100 cuts the MdAPE by approximately 50\%. For NFTY-5K, it's performance is similar to SLoPS' for the single-threaded \NFs but reduces MdAPE by at least 90\% for the multi-threaded \NFs.  


\begin{figure}[t!]
    \centering
    \begin{subfigure}[b]{0.48\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{fig/comp_all_5000_barchart_internet.png}
    \caption{\label{fig:int-5k}}
\end{subfigure}
\begin{subfigure}[b]{0.48\columnwidth}
    \centering
    \includegraphics[width=\columnwidth]{fig/comp_all_100_barchart_internet.png}
    \caption{\label{fig:int-100}  }
\end{subfigure}
\caption{ (a) Comparing SLoPS-5K and \syslarge in internet experiments with an optimized sender and unoptimized \NF. (b) Same setting as (a), but now comparing NFTY-100 and SLoPS-100.}
\Description[\sys comparison with baseline in the Internet setting]{(a) Comparing SLoPS-5K and \syslarge in internet experiments with an optimized sender and unoptimized \NF. (b) Same setting as (a), but now comparing NFTY-100 and SLoPS-100.}
\end{figure}

\subsection{Case Study: \sys against Commercial NF in the Cloud} \label{sec:aws}
Having tested \sys in the lab and in the Internet we aim to investigate whether our results generalize beyond open-access \NFs and in-house deployments. To this end, we use \sys to calculate the capacity of the Fortinet next-generation firewall\cite{fortinet} which is a closed-source and commercial NF.

\myitem{Cloud setup:} We deploy the Fortinet firewall in the AWS US East cluster on an AWS c4.large instance type in front of a private subnet which was the recommended instance type by the vendor. Thus,  all traffic entering the subnet passes through the firewall as we show in Figure\ref{fig:aws-setup}. We have configured the firewall to use its default attack detection profiles for all UDP traffic. We find the ground truth processing capacity to be 62738 pps.
We measure the ground truth using a local node within AWS by flooding the NF and measuring the received rate at the receiver. We found that when we flood the NF, the receiver constantly receives packets at a rate of 62738 pps, and the remaining packets are dropped at the NF.
We use our Clemson Cloudlab node to probe the firewall using UDP traffic to implement \syslite. Observe that traffic from Clemson to the AWS nodes is forwarded through the public Internet and, thus is subject to cross-traffic.

We find that \syslite can accurately estimate the processing capacity of the Fortinet firewall within 7\% error. The spread in the error is high, which might be due to the the noise from use of a VM  of either \NF or the receiver node~\ref{fig:aws}. This shows that given an unknown NF with unknown deployment, \sys can accurately estimate its processing capacity.

% \maria{How do we measure ground truth here? Did we 'get caught'?}

==> e2e.tex <==
%\section{End-to-end view of \sys}  %\setkeys{
%}{} Bringing it all together}

%\vyas{Use some preamble like  this: Combining the insights from the previous section, next we present an end-to-end overview of the \sys framework to tackle the Relaxed \NFCR problem.} 


%Consider an attacker that aims to DDoS an enterprise network. To calculate the resources she needs, the attacker aims at profiling the firewall that the enterprise deploys at its edge.
%The attacker is willing to send up to $3000$ packets to prevent the target network from detecting her attack and upgrading her infrastructure. 
\remove{
\myitem{Two-sided attack example} 
Assume that our attacker uses \sys and has infected a host in the targeted network. 
The attacker sends $3000$ packets as fast as she can to instantly stress the \NF. 
She sends the same 5-tuple to avoid her packets being re-order in the Internet path before they reach the receiver.
Upon reception, the infected host captures those $3000$ packets and stores their timestamps.
Since the attacker relies on the time measurements, she ensures that these are fine-grained and minimum unaffected by server configuration such as batching. 
The attacker then calculates the inter-arrival times between these packets and uses it to calculate the firewall's capacity. To that end, the attacker uses a function $F$, which first selects a window of the most reliable measurements and reports the mean. 



\myitem{Single-sided attack example} 
Assume that our attacker uses \sys and has no infected host.
The attacker again sends $3000$ packets of the same 5-tuple, but this time at one of the IPs that are assigned to the enterprise.
She again sends those packets at once, but she sets the Time To Live (\ie one of the IP header fields) of a subset of the sent packets to a lower value than the default.
By doing so, the attacker triggers the generation of some error message from a router in the path from the NF to the destination IP. Most importantly, as the TTL is an IP header, the triggering can be applied to any packet type that the target \NF processes. The attacker minimizes the number of such packets to reduce the stress on the device. 
The attacker captures the error messages, stores their timestamps, and calculates the time difference between arrivals.
These data is fed to $F'$ to calculate the capacity.
}
